Math Operation Embeddings for Open-ended Solution Analysis and Feedback

Feedback on student answers and even during intermediate steps in their solutions to open-ended questions is an important element in math education. Such feedback can help students correct their errors and ultimately lead to improved learning outcomes. Most existing approaches for automated student solution analysis and feedback require manually constructing cognitive models and anticipating student errors for each question. This process requires significant human effort and does not scale to most questions used in homework and practices that do not come with this information. In this paper, we analyze students' step-by-step solution processes to equation solving questions in an attempt to scale up error diagnostics and feedback mechanisms developed for a small number of questions to a much larger number of questions. Leveraging a recent math expression encoding method, we represent each math operation applied in solution steps as a transition in the math embedding vector space. We use a dataset that contains student solution steps in the Cognitive Tutor system to learn implicit and explicit representations of math operations. We explore whether these representations can i) identify math operations a student intends to perform in each solution step, regardless of whether they did it correctly or not, and ii) select the appropriate feedback type for incorrect steps. Experimental results show that our learned math operation representations generalize well across different data distributions.

==> experiments_j.tex <==
\section{EXPERIMENTS}
\zw{jw wrote this para} \ml{we need to merge this with the above. I think let's go with 5.1 - data, 5.2 - math operation classification, 5.3 - feedback classification. Then, in 5.2, we organize as 5.2.1 methods and metrics (seems hard to use ``baselines'' here since i'm not sure there are standard baselines for these tasks), 5.2.2 experimental setup, and 5.2.3 results and discussion. We then repeat in 5.3, only that now our descriptions are much shorter - we only detail what's different from 5.2.}
We now demonstrate the effectiveness of our proposed approach over various baselines on XXX dataset. we perform 2 experiments, one on math operation classification and one on feedback classification. 


\subsection{Dataset}
\zw{jw wrote this subsection} \ml{see what i wrote about notation in section 4.}
We represent the math equations as a sequence of math symbols. We denote $\vx_1^{(i)} = \{x_t\}_{t=1}^{T_1}$ and $\vx_2^{(i)} = \{x_t\}_{t=1}^{T_1}$ as the $i$-th solution step before and after taking a particular math operation $y$, respectively, where $x_t\in V$ is a math symbol in the math vocabulary set $V$. \ml{maybe an example would be good here, although ideally we should provide such an example in the intro using a figure.} Further, each step may be associated with a feedback $w$. \ml{lets call feedback $y$? operations are referred to as $z$.}
Table XXX gives an example entry of our dataset. 

\zw{copied from a subsequent paragraph} We further separate the data into three parts, \texttt{OK} steps that are deemed to be correct according to the specified solution template, \texttt{BUG} steps that contain erroneous solutions that fit anticipated errors built into Cognitive Tutor and the system can automatically recognize these errors and deploy the corresponding feedback, and \texttt{ERROR} steps where student commit unanticipated errors that the system does not recognize. 
\zw{TODO: expand, i.e., dataset stat, general preproc steps}

\subsection{Baseline} \ml{this needs changing but it's hard to figure out exactly how to change before we know what the methodology section looks like.} \zw{jw wrote this subsection} 
We implement two simple classification baselines $f_\Theta$ and $f_\Phi$, both of which are widely used in NLP classification tasks such as sentiment analysis [CITE]. 

{\bf RNN baseline.} Here, $f_\Theta$ contains a uni-directional gated recurrent neural network (GRU) [CITE] as the main feature extractor, together with input embedding and a linear classifier. For example, for the step classification task where the target variable is $\rvy$, we have
\begin{align*}
    \widehat{y} &= \underset{y}{{\rm argmax}}\, f_\Theta(\vx_1, \vx_2)\,,\\
    f_\Theta &= {\rm softmax} 
    \left(\rmV^\top [\vh_{T_1}; \vh_{T_2}] + \rvb \right)\,,\\
    \vh_t &= {\rm GRU}_\theta (\ve_t, \vh_{t-1})\,,\\
    \ve_t &= \rmW^\top {\rm onehot}(x_t)\,,
    % \widehat{y} &= \underset{y}{{\rm argmax}}\,\, {\rm softmax} 
    % \left(\rmV^\top [\vh_{T_1}; \vh_{T_2}] + \rvb \right)
\end{align*}
where $\vh_t\in\mathbb{R}^{D}$ is a D-dimensional state vector in GRU and $\ve_t\in\mathbb{R}^{M}$ is an M-dimensional math token embedding. $\rmW\in\mathbb{R}^{|V|\times M}$, $\rmV\in\mathbb{R}^{D\times |\vy|}$, and $\theta$ comprise the parameter $\Theta$ where $|\cdot|$ denotes the cardinality function. The optimization objective is to accurately predicts $y$ given $\vx_1$ and $\vx_2$. Formally, we have
\begin{align*}
    \widehat{\Theta} =
    \underset{\Theta}{{\rm argmin}}\, \mathbb{E}_{\vx_1,\vx_2,y\sim\mathcal{D}} [-{\rm log} f_\Theta(\vx_1,\vx_2)]\,,
\end{align*}
where $\mathcal{D}$ denotes the empirical data distribution. The baseline and its optimization objective for the feedback classification is the same as above, except that the target variable changes from $y$ to $w$. 

{\bf CNN baseline.} Here, $f_\Phi$ contains a 2D convolutional neural network (CNN) as the main feature extractor with the same embedding and classifier architecture as in the previous baseline. Concretely,
\begin{align*}
    \widehat{y} &= \underset{y}{{\rm argmax}}\, f_\Phi(\vx_1, \vx_2)\,,\\
    f_\Phi &= {\rm softmax} 
    \left(\rmV^\top [\vh_{1}; \vh_{2}] + \rvb \right)\,,\\
    \vh &= {\rm max\_pool}({\rm CNN}_\phi ([\ve_1,\cdots,\ve_{T_1}]))\,,\\
    \ve_t &= \rmW^\top {\rm onehot}(x_t)\,,
    % \widehat{y} &= \underset{y}{{\rm argmax}}\,\, {\rm softmax} 
    % \left(\rmV^\top [\vh_{T_1}; \vh_{T_2}] + \rvb \right)
\end{align*}
where ${\rm CNN}_\phi$ represents a 2D CNN and ${\rm max\_pool}$ is a 1D max pooling operator. Combined, they return a fixed dimensional feature vector $\vh$ that represents a math equation denoted as $\vh_1$ and $\vh_2$,respectively.  

For both experiments, we perform 5-fold cross validation on the dataset and train our baseline with Adam [CITE] optimizer with learning rate $0.001$. $D=M=512$. 
\zw{variable names can be changed and unified later}


\subsection{Math Operation Classification}
\zw{jw wrote this subsection}
This experiment aims to validate our approach's capability in correctly recognizing the step, i.e., multiplication, subtraction, and division, that a student takes in a particular derivation to solve a problem. Thus, each data point in this experiment is a tuple consisting of $(\vx_1, \vx_2, y)$.

\subsubsection{Experiment Setup}
TODO: label preprocessing etc., model setup etc

\zw{copied from a subsequent paragraph} We test our math operation representation learning methods on the \texttt{OK} subset via 5-fold cross validation, i.e., training on $80\%$ of data points to learn the math operation representations and test the learned representations on the remaining $20\%$ of data points. We also experiment with three additional experimental settings to test the generalizability of the learned representations to transfer: First, we use synthetically generated data as the training set to evaluate generalizability from synthetic data to real data. Second, we use the \texttt{BUG} and \texttt{ERROR} data subsets as test sets to evaluate generalizability from correct steps to incorrect steps. Third, we further divide the data into different difficulty levels for the corresponding questions (six levels, from $0$ to $5$) to evaluate generalizability across different difficulty levels.

\subsubsection{Results}
Table XXX compares the classification accuracy of our method with baseline. We see that our method achieves higher classification accuracy and that the improvement is statistically significant. This result suggests that explicitly encoding math equations as trees is beneficial, and that pre-training on large-scale math equation corpus leads to further performance improvements. 

Table XXX presents qualitative examples that further illustrates the performance of our method compare to baselines. In all these examples, our method can accurately identify the correct step, whereas the baseline fails to do so. This is because ... \zw{may nor may not need these qualitative examples; write here as a placeholder}


\subsection{Feedback Prediction}
\zw{copied from a subsequent paragraph} In this experiment, we use only the \texttt{BUG} subset of the entire dataset. We perform cross validation on this subset to evaluate the generalizability of feedback to new questions and difficulty levels that are not included in the training set. 

We used the ``Cog Tutor 2010 Equation Solving (sch\_bd1124)'' dataset accessed via DataShop \cite{pslc}. 

Overview of all experiments we are going to run:
\begin{itemize}
    \item Predicting math operation used in student solutions
    \begin{itemize}
        \item We break down the entire dataset into a series of \emph{data points}: each data point corresponds to a single step in a student's solution process to an equation solving question through applying one of the following math operations: add, subtract, combine, \ldots. We separate the data into three parts, \texttt{OK} steps that are deemed to be correct according to the specified solution template, \texttt{BUG} steps that contain erroneous solutions that fit anticipated errors built into Cognitive Tutor and the system can automatically recognize these errors and deploy the corresponding feedback, and \texttt{ERROR} steps where student commit unanticipated errors that the system does not recognize. 
        
        
        \item We test our math operation representation learning methods on the \texttt{OK} subset via 5-fold cross validation, i.e., training on $80\%$ of data points to learn the math operation representations and test the learned representations on the remaining $20\%$ of data points. We also experiment with three additional experimental settings to test the generalizability of the learned representations to transfer: First, we use synthetically generated data as the training set to evaluate generalizability from synthetic data to real data. Second, we use the \texttt{BUG} and \texttt{ERROR} data subsets as test sets to evaluate generalizability from correct steps to incorrect steps. Third, we further divide the data into different difficulty levels for the corresponding questions (six levels, from $0$ to $5$) to evaluate generalizability across different difficulty levels.
    \end{itemize}
    \item Predicting feedback in ``buggy'' solution steps
    In this experiment, we use only the \texttt{BUG} subset of the entire dataset. We perform cross validation on this subset to evaluate the generalizability of feedback to new questions and difficulty levels that are not included in the training set. 
\end{itemize}
